Solving Max-Min Fair Resource Allocations Quickly on Large Graphs

We consider the max-min fair resource allocation problem. The best-known solutions use either a sequence of optimizations or waterfilling, which only applies to a narrow set of cases. These solutions have become a practical bottleneck in WAN traffic engineering and cluster scheduling, especially at larger problem sizes. We improve both approaches: (1) we show how to convert the optimization sequence into a single fast optimization, and (2) we generalize waterfilling to the multi-path case. We empirically show our new algorithms Pareto-dominate prior techniques: they produce faster, fairer, and more efficient allocations. Some of our allocators also have theoretical guarantees: they trade off a bounded amount of unfairness for faster allocation. We have deployed our allocators in Azure's WAN traffic engineering pipeline, where we preserve solution quality and achieve a roughly $3\times$ speedup.

==> texfiles/design_v3.tex <==
\newpage
\newpage
\newpage

\section{New Design}

Preludes:

1) Definition of Max-Min fairness

2) Model that says how our algorithms apply to different problems.
E.g., multiple-resources such as `links'
demands ask for a certain rate $d$
demands can be satisified by allocating some fraction $t$  along all the links on a 'path'  (path = group of resources which must be allocated together, some cases require different amount at different resources such as say 20\% CPU and 50\% memory but require all of them simultaneously)
a demand can be assigned resources along multiple possible 'paths' (e.g., a map-reduce job can be assigned resources at any machine in the cluster)

Edit FeasibleFlow throughout to be something from the model.

\section{Max-Min Fair Resource Allocators}
Here, we discuss two kinds of novel allocators that advance the state-of-the-art in allocating multiple resources in a max-min fair manner.


\subsection{One-shot Optimizations}
\label{s:oneshotopts}

\noindent{\bf Overview: }
It is easy to think of max-min fair resource allocation as an optimization with a prioritized list of objectives. 
That is, first maximize the smallest allocation. 
Then, maximize the second smallest allocation and so on. 
This intuition naturally leads to solving a sequence of linear optimization problems~(LPs) to compute the max-min fair allocations~\cite{danna,swan}.
In prior work, the number of LPs to solve can be as many as the number of unique resources~\cite{danna}~(e.g., the number of edges in a network or machines in a cluster).
We will first show that such a prioritized list of objectives can be linearized so that we may solve one optimization instead of a (long) sequence.
Although this single optimization is analytically interesting, we will show that optimizations with such a linear combined objective encounter double precision errors, require a sorting network in the formulation and consequently are slower in practice.

Next, we consider an approximate variant of max-min fairness from SWAN~\cite{swan} which uses geometric binning.
Given a user-specified parameter $\alpha$ (e.g., $\alpha=2$ in~\cite{swan}), SWAN uses many fewer LPs to guarantee that allocations are never more than $\alpha\times$ away from the optimal fair values. 
Larger $\alpha$ leads to more unfairness but requires fewer LPs.\footnote{The number of LPs is $\lg_\alpha Z$ where $Z$ is the ratio between the largest and the smallest rate.}
SWAN has been in production at Microsoft for many years now~\cite{onewan}. 

A key contribution in our work is to combine the above two ideas. 
That is, we will show that this approximate max-min fairness can be linearized, i.e., converted to a one-shot optimization.
Our combination is novel, has the same worst-case fairness guarantees as SWAN but, by linearizing at the granularity of bins, no longer encounters double precision issues, needs no sorting network and is empirically faster. 
We also reason intuitively why this one-shot optimization will be fundamentally smaller and faster than SWAN’s sequence of optimizations.
We will discuss results from deploying this algorithm in production at a large cloud provider. 


Recall the max-min fair definition in the model. Here, we will consider a simple case wherein all demands are treated equally fairly (i.e., not weighted max-min fair) and resource requirements are the same at different resources (e.g., rate on different network links). Generalizing either of these aspects is direct and we briefly discuss how to do so in~\S\ref{}.

\vspace{0.05in}
\noindent{\bf Max-min fair as a sequence of LPs:}
If there are $n$ demands and $t_i$ are the sorted max-min fair rates, then max-min fair allocation can be computed using $n$ LPs wherein the $i^{\mbox{th}}$ LP in the sequence maximizes the $i^{\mbox{th}}$ smallest rate. That is:

{\small
	\begin{align}
		\label{eq:seq-max-min-flow}
		\mbox{\sf MaxMin}_{i}(\mathcal{E}, \mathcal{D}, \mathcal{P}, \mathcal{Q}, \mathcal{R}) \triangleq & \arg\max~~ t_{i} \\
		\mbox{s.t.} & \quad t_{i} = \text{\sf (i)-th smallest rate} (\mathbf{f}), \nonumber \\ 
		 & \hspace{-3mm} (t_1, \dots, t_{i-1}) \in \mbox{\sf MaxMin}_{i-1}(\mathcal{E}, \mathcal{D}, \mathcal{P}, \mathcal{Q}, \mathcal{R}), \nonumber \\
		 & \hspace{-3mm} \mathbf{f} \in {\sf FeasibleFlow}(\mathcal{E}, \mathcal{D}, \mathcal{P}, \mathcal{Q}, \mathcal{R}).\nonumber
	\end{align}
}
\srikanth{what are Q and R? needed? re-verify.}
Prior work offers similar formulations and we use this as only the beginning point.

\vspace{0.05in}
\noindent{\bf One-shot Optimal Max-min fair:}
To reformulate Eqn.~\ref{eq:seq-max-min-flow} as a single optimization, we make two changes which are shown in bold red below. 
First, we use a linear weighted objective where the weight on a rate decreases based on their rank in the sorted order; that is, the objective incentivizes increasing the smaller rates.  
Next, we use a sorting network~\cite{ffc,pretium} to determine the sorted order of rates. 
Since Eqn.~\ref{eq:seq-max-min-flow}  only maximizes the next smallest rate in each LP, no explicit sorting was required but the one-shot nature of our new LP requires sorting to weight each allocation appropriately.

{\small
	\begin{align}
		\label{eq:opt_max_min_flow}
		\mbox{\sf OneShotOpt}(\mathcal{E}, \mathcal{D}, \mathcal{P}, \mathcal{Q}, \mathcal{R}) ~ \triangleq & ~ \arg\max_{\mathbf{f}} \textcolor{red}{\sum_{i=1}^{n} \epsilon^{i-1}} t_i \\
		\mbox{s.t.} & ~~ \textcolor{red}{({t_1},\dots,{t_n}) = \text{\sf sorted rates} (\mathbf{f})},\nonumber \\
		& \hspace{-3mm}\mathbf{f} \in {\sf FeasibleFlow}(\mathcal{E}, \mathcal{D}, \mathcal{P}, \mathcal{Q}, \mathcal{R}).\nonumber
	\end{align}
}

We can prove that {\sf OneShotOpt} leads to a max-min fair rate allocation. Specifically,
\begin{theorem}
	\label{th:epsilonOneShot}
	There exists a (small enough) value of $\epsilon$ for which the optimization in~\eqnref{eq:opt_max_min_flow} yields the same max-min fair rate allocations as the sequence of optimizations shown in~\eqnref{eq:seq-max-min-flow}.
\end{theorem} 

\begin{proof}[Proof Sketch]
	Intuitively, by definition of max-min fairness, the smallest rate assigned by~\eqnref{eq:opt_max_min_flow} cannot be larger than the the smallest rate assigned by~\eqnref{eq:seq-max-min-flow}. 
	Furthermore, the optimal max-min fair rate vector, say ${\textbf{t^*}}$, is a feasible solution to~\eqnref{eq:opt_max_min_flow}. 
	Thus, the solution from~\eqnref{eq:opt_max_min_flow} say ${\bf t^\dag}$ must satisfy: $\sum_i \epsilon^{i-1} t^\dag_i \geq \sum_i \epsilon^{i-1}t^*_i$. 
	If the smallest rate in ${\bf t^\dag}$ happens to be less than its counterpart in ${\bf t^*}$, then the other rates will have to increase by at least a ratio of $\frac{1}{\epsilon}$. 
	Thus, as $\epsilon \rightarrow 0$, the smallest rates must match. 
	Inductively, the same argument holds for each index.  
\end{proof}

We note a few practical concerns for {\sf OneShotOpt}. 
First, as the proof shows, we must use small values of $\epsilon$ to ensure optimality but, if the smallest weight, $\epsilon^n$, is too small, we will encounter double precision errors~\cite{}.
Thus, especially when there are many demands (large $n$), this formulation has to sacrifice optimality to be feasible.
Next, the sorting network to order the rates so as to give them the appropriate weights, requries up to $O(nlog^2(n))$ additional constraints.
Taken together, we will show that {\sf OneShotOpt} is only feasible on very small graphs.





\vspace{0.05in}
\noindent{\bf One-shot Geometric Binner:}
Inspired by SWAN~\cite{swan}, Eqn.~\ref{eq:seq-approx-max-min-flow} shows a sequence of LPs with key parts in red. 
%
{\small
	\begin{align}
		\label{eq:seq-approx-max-min-flow}
		\mbox{\sf ApproxMaxMin}_{i}(\mathcal{E}, \mathcal{D}, \mathcal{P}, \mathcal{Q}, \mathcal{R}) \triangleq & \arg\max \sum_i t_{i} \\
		\mbox{s.t.} & \quad \textcolor{red}{t^i_{k} \leq U ~ \alpha^i} ~ \forall k, \nonumber \\ 
		 & \hspace{-3mm} \textcolor{red}{t^i_k  = t^{i-1}_k ~~ \mbox{if} ~~ t_k^{i-1} < U \alpha^{i-1}}, \nonumber \\
		 & \hspace{-3mm} \mathbf{f} \in {\sf FeasibleFlow}(\mathcal{E}, \mathcal{D}, \mathcal{P}, \mathcal{Q}, \mathcal{R}).\nonumber
	\end{align}
}
%
As shown, the $i^{\mbox{th}}$ LP allocates rate {\em only up to} $\alpha^i U$ and any demand that does not fully use the allocation from the previous LP will be frozen to its previous allocation. Here, $U$ is some minimum rate and $\alpha$ is a parameter such as $2$. While clearly each LP in the sequence allocates rates unfairly, the unfairness is bounded since each LP allocates rates only within a {\em bucket} and one can prove that demands are promoted to the next LP in the sequence only if their max-min fair rates would be at least as large as $\alpha^i U$.  Note that the number of LPs in this format will be $\log_\alpha Z$ where $Z$ is the ratio of the maximum to the minimum rate.

\begin{figure}[th!]
	\centering
	\includegraphics[width=0.8\linewidth]{figs/methods/geometric_binning_example.pdf}
	\caption{\textbf{Geometric Binning: } Approx. one-shot max-min fair allocations.}
	\label{f:geo-binning-example}
\end{figure}
\autoref{f:geo-binning-example} shows the key idea behind our one-shot geometric binner.  
If we think of each allocation as being the sum of contributions from different, geometrically sized, bins, we can use $\epsilon$-weighting per bin and incentivize allocating more flow to the smaller bins.
The resulting formulation is:

{\small
	\begin{align}
	\label{eq:new_geobinning}
\mbox{\sf GeoBinning}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P}) \triangleq & \arg\max_{\mathbf{f}} \sum_{k \in \mathcal{D}}\sum_{\mbox{bins} ~ b} \epsilon^{b-1} f_{kb}\\
\mbox{s.t.} \quad & f_{k} = \mathcal{U} + \sum_{\mbox{bins} ~ b} f_{kb} \quad \forall k \in \mathcal{D} \nonumber\\
% & f_{k0} = \mathcal{U} \quad \forall k \in \mathcal{D} \nonumber\\
& f_{kb} \le U ~ (\alpha^{b} - \alpha^{b-1}) \quad \forall k \in \mathcal{D}, ~ b \in \{1\dots\} \nonumber\\
&\mathbf{f} \in {\sf FeasibleFlow}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P},\mathbbm{1},\mathbbm{1}),\nonumber 
\end{align}
}

We note a few properties of~\eqnref{eq:new_geobinning}.
\begin{Itemize}
\item
The method above can apply to a variety of bin choices and not just the geometrically increasing bins used here.
Inspired by similar intuition to equi-depth binning in databases, we will show that choosing bin boundaries differently can reduce the approximation error in~\S\ref{}.
\item
Next, we can prove that using the same (geometric) bins as SWAN~\cite{swan} yields the same approximation guarantee: specifically {\sf GeoBinning} ensures that the allocation for any demand will be within an $\alpha$ ratio of the optimal max-min fair rate. Specifically, we show:
\begin{theorem}
	\label{th:binFilling}
	For any choice of bins, \eqnref{eq:new_geobinning} will assign resources to a demand $k$ in a bin $b$ only if demand $k$ has been assigned the full rate from all of the larger-weighted bins. \end{theorem} 
\begin{proof}[Proof Sketch]
 Assume otherwise. That is, some demand $k$ has received non-zero allocation in some bin $b$ while its allocation in some other bin $i$ (where $i<b$) is not full. Then, we can move some $\delta$ amount of flow from bin $b$ to bin $i$ without violating any of the constraints and improve the objective value\footnote{Bin $i$ has a larger weight because $\epsilon <1$ and smaller indexed bins have higher weights}.
\end{proof}
Using Theorem~\ref{th:binFilling} alongside Theorem~\ref{th:epsilonOneShot} ensures that the allocation of Eqn.~\ref{eq:new_geobinning} will match SWAN.
\item As with SWAN~\cite{}, a user can vary $\alpha$ to trade-off an approximation in fairness for faster solver time.
\item 
Note that the number of bins is often much smaller than the number of demands and so appropriately small values can be chosen $\epsilon$ without running into double precision errors unlike the case of~\eqnref{eq:opt_max_min_flow}.
\item 
Similarly, unlike Eqn.~\ref{eq:opt_max_min_flow}, Eqn.~\ref{eq:new_geobinning} requires no sorting constraints.
\item
The number variables is approximately the same between this one-shot optimization and the total among all of the sequence of optimizations in Eqn.~\ref{eq:seq-approx-max-min-flow}; Eqn.~\ref{eq:new_geobinning} has one variable per demand and bin whereas Eqn.~\ref{eq:seq-approx-max-min-flow} uses one LP per bin and one variable per demand in each LP.
The key difference is that we can now run one LP which is likely to be faster than running (about the same optimization) in many sequential steps.
Thus, we reason that the one-shot optimization will be faster in general and our empirical findings verify this reasoning.
\end{Itemize}

\subsection{Multi-path Waterfilling}
\label{s:genwaterfilling}
Here, we generalize the classical waterfilling algorithm to allocate multiple resources in a max-min fair manner. Compared with~\S\ref{s:oneshotopts}, the techniques here do not solve optimizations but are parallelizable combinatorial algorithms. In general, these algorithms have better empirical performance but weaker fairness guarantees.

Waterfilling is a simple and well-known method to share a single resource in a max-min fair manner between multiple demands: iteratively allocate the remaining resource *fairly* among the remaining demands while, in each iteration, any demand that receives its full allocation does not proceed to the next iteration. 
This method directly extends to multiple resources in the special case where each demand requires resources on {\em exactly one path} (that is, all the resources in a given set). Intuitively, one can visit resources in each iteration in the order of their smallest fair share and allocate resources to demands based on the fair share at their tightest resource. See~\autoref{alg:one_path_wt_waterfilling} for the pseudocode\footnote{To simplify the algorithm, we model demand constraints by adding one virtual edge per demand whose capacity is equal to the flow's demand.}. Furthermore, this method is parallelizable by independently considering resources which do not have any demands in common.


{\small
\RestyleAlgo{ruled}
\begin{algorithm}[t!]
	\DontPrintSemicolon
	\LinesNumbered
	\caption{Waterfilling algorithm to compute weighted max-min fairness on one path.}
	\label{alg:one_path_wt_waterfilling}
	\KwIn{$\weightedroutingmatrix_{M \times K}$: $\weightedroutingmatrix[m,k]$ is the weight of demand $k$ on link $m$.}
	\KwIn{$\capacity_{M \times 1}$: link capacities.}
	\KwOut{$\rate_{K \times 1}$: max-min rate of each demand.}
	
	$\setactiveflows \leftarrow \mathbbm{1}_{|K| \times 1}$ \algcomment{set of active demands}\;
	$\rate_{K \times 1} \gets 0$ \algcomment{initial rates} \;

	\While{$|\setactiveflows| > 0$}{
		$N \gets \weightedroutingmatrix \setactiveflows$ \algcomment{total weight per link.}\;
		$\fairshare \gets \frac{\capacity}{N}$ \algcomment{vector division, fairshare per link.}\;
		$l \gets \mathop{\mathrm{arg\,min}_e} \fairshare_e$ \algcomment{link with minimum fair share}\;
		\For{$f:  \weightedroutingmatrix[l, f] > 0$  \algcomment{demands on link $l$}}{
			$\rate_f \gets \fairshare_l \weightedroutingmatrix[l, f]$ \algcomment{Fix rate by tightest}\;
		}
		\algcomment{deduct capacities at all links allocated above}\;
		$\setactiveflows \gets \setactiveflows \setminus \{f:  \weightedroutingmatrix[l, f] > 0\}$	\algcomment{update active set}\;
	}
\Return{$\rate$}
\end{algorithm}
}

Waterfilling does not generalize however to the case when a demand can be allocated along multiple paths because, intuitively, the global max-min fair allocation need not be locally max-min fair, i.e., max-min fair at each resource. \autoref{f:example:water} shows such an example wherein the blue demand that has access to more paths must receive a locally unfair share on the common path.

\renewcommand{\arraystretch}{1.1}
\begin{figure}[t]
	\centering
	\label{f:example:water}
	\subfigure[Global max-min fair is not the same as local (per-link) max-min fair]{\includegraphics[width=1.0\linewidth]{figs/max-min-fair-algorithm-example.pdf}}
	
	\subfigure[Illustrating Adaptive Waterfilling]{
%		\begin{table}
%			\centering
			\begin{tabular}{l|cccccc}

				& \multicolumn{6}{l}{\bf \# iteration $t\longrightarrow$}\\\hline

				$\theta^1_1$ 	& $\frac{1}{2}$ & $\frac{3}{5}$ 	& $\frac{7}{11}$ 	& $\frac{15}{23}$ 	& $\frac{31}{47}$ 	& $\frac{63}{95}$ \\

				$\theta^2_1$ 	& $\frac{1}{2}$ & $\frac{2}{5}$ 	& $\frac{4}{11}$ 	& $\frac{8}{23}$	& $\frac{16}{47}$	& $\frac{32}{95}$\\

				$\theta^1_2$ 	& $1$ 			& $1$				& $1$ 			 	& $1$				& $1$				& $1$\\


				$f^1_1$ 		& $\frac{1}{2}$ & $\frac{1}{2}$		& $\frac{1}{2}$ 	& $\frac{1}{2}$		& $\frac{1}{2}$		& $\frac{1}{2}$\\


				$f^2_1$ 		& $\frac{1}{3}$ & $\frac{2}{7}$		& $\frac{4}{15}$ 	& $\frac{8}{31}$	& $\frac{16}{63}$	& $\frac{32}{127}$\\


				$f^1_2$ 		& $\frac{2}{3}$ & $\frac{5}{7}$		& $\frac{11}{15}$ 	& $\frac{23}{31}$	& $\frac{47}{63}$	& $\frac{95}{127}$\\

			\end{tabular}
	
%		\end{table}
	}
	\caption{Example.}
\end{figure}
\renewcommand{\arraystretch}{1}

\vspace{0.05in}
\noindent
{\bf ApproxWaterfiller: } Simply have a sub-flow on each path. All sub-flows share the demand constraint edge so total allocation is still constrained. Apply algorithm~\ref{alg:one_path_wt_waterfilling} per subflows. 
This would not have global max-min fairness but can be efficient and we make a few more changes to increase parallelizability. Specifically, see algorithm~\ref{alg:one_path_approx_wt_waterfilling}.

{\small
\RestyleAlgo{ruled}
\begin{algorithm}[t]
	\DontPrintSemicolon
	\LinesNumbered
	\caption{Our Approx. Max-Min Fair Waterfiller.}
	\label{alg:one_path_approx_wt_waterfilling}
	\KwIn{$\weightedroutingmatrix_{M \times K}$: sub-flow weights where $\weightedroutingmatrix[m,k]$ shows the weight of sub-flow $k$ on link $m$.}
%	\KwIn{$\routingmatrix_{M \times K}$: routing matrix where where $\routingmatrix[m,k] = 1$ if sub-flow $k$ uses link $m$, otherwise $=0$}
	\KwIn{$\capacity_{M \times 1}$: link capacities.}
	\KwOut{$\rate_{K \times 1}$: max-min rate of each sub-flow.}
	
	${\rate} \gets \infty_{K \times 1}$ \algcomment{initial max-min rate set to $\infty$}\;
	$N \gets \weightedroutingmatrix \mathbbm{1}_{K \times 1}$ \algcomment{weight of sub-flows per link}\;
	$\set{L} \gets \mathop{\mathrm{arg\,sort}}\frac{\capacity}{N}$ \algcomment{sort links in ascending order}\;
	\For{$l \in \set{L}$}{
		$\setflows_l \gets \{ f: \weightedroutingmatrix[l, f] > 0 \}$ \algcomment{sub-flows on link $l$}\;
		$\hat{\rate} \gets 0_{|\setflows_l|}$ \algcomment{initial fair share for each sub-flow}\;
		\While{$\setflows_l \neq \emptyset$}{
			\tcc{compute link and sub-flow fair shares.}
			$\fairshare \gets \frac{\capacity_l}{\sum \weightedroutingmatrix[l, \setflows_l]}$ \;
			$\hat{\rate}_{\setflows_l} = \fairshare \weightedroutingmatrix[l, \setflows_l]$ \;
			\tcc{compuate set of flows requesting less than fair share}
			$\set{U} \gets \{i:i \in \setflows_l \And \rate_i < \hat{\rate}_i\}$ \;
			\uIf{$\set{U} = \emptyset$}{
				\tcc{if all the sub-flows are requesting more than fair share, set their rate and break.}
				$\rate_{\setflows_l} \gets \hat{\rate}_{\setflows_l}$ \;
				$break$ \; 
			}\Else{
				\tcc{otherwise, remove the sub-flows requesting less and recompute the fair share.}
%				$\hat{\rate}_{\set{U}} \gets \rate_{\set{U}}$ \;
				$\capacity_l \gets \capacity_l - \sum \rate_{\set{U}}$ \;
				$\setflows_l \gets \setflows_l \setminus \set{U}$\;
			}
		}
	}
	\Return{$\rate$}
\end{algorithm}
}

\vspace{0.05in}
\noindent
{\bf AdaptiveWaterfiller: } Adapt the proportions on each sub-flow in a way that steers more demand to paths where more allocation was obtained.
More specifically, we compute an initial set of flow assignments for each subflow using the {\sf ApproxWaterfiller} with path proportions set equally and 
iteratively update the proportions as: 
$\theta^p_{k} (t + 1) = \frac{f^{p}_{k} (t)}{f_{k}(t)}$ where $f^{p}_{k}(t)$ is the allocation for demand $k$ on path $p$ at iteration $t$ and 
$\theta$ is the multiplier for the underlying weights.
The algorithm converges when \cradd{$\theta^{p}_{k} (t+1) = \theta^{p}_{k}(t)$}.  
We can prove that adapting the proportions leads to better global max-min fairness. 
Specifically, we define the notion of bandwidth bottleneck.
We say that a flow \cradd{$f_k$} is \emph{bandwidth bottlenecked} in the multi-path setting if: (i) Each of its subflows \cradd{$f^{p}_{k}$} is bottlenecked on some link $l$, and (ii) \cradd{$f_k \ge f_j$, $\forall f_j$} for all demands $j$ that have a subflow on any such bottleneck link $l$.
With this definition in place, we can show that: (see~\S\ref{sec:proof_bottleneck} for the proof).

\begin{theorem}\label{T:bandwith_bottleneck}
	{\em If} the adaptive waterfiller converges, it converges to a bandwidth bottlenecked point in the space of feasible flow-assignments. 
\end{theorem}

We also show the max-min fair rate allocation is bandwidth bottlenecked (see~\S\ref{sec:additional_results_waterfilling}), although not all bandwidth-bottlenecked rate allocations are max-min fair. 
Moreover, the set of bandwidth-bottlenecked allocations is {\em significantly} smaller than the feasible set.
We can also show that (see~\S\ref{sec:additional_results_waterfilling} for proof) the adaptive waterfiller converges when it finds a bandwidth-bottlenecked rate allocation (\ie it does not iterate thereafter). 
Although we do not have a theoretical characterization of convergence, we find empirically the method converges within $5$ iterations (\secref{s:conv-sens-analys}).

In summary, adaptive waterfiller produces rate assignments that are feasible, and belong to a constrained set that contains the optimal max-min fair rates.
It is slower than approximate waterfiller because it changes proportions and iterates, but is faster than geometric binner, so we include it as a standalone allocator. 
Users can tune the number of iterations to trade-off between fairness and speed.



==> texfiles/gbproof.tex <==
\begin{lemma}
	\label{lemma:gb:1}
	\cradd{The optimal solution of GB (\eqnref{eq:geobinning}) only assigns resources from bin $b$ to a given demand $k$ if demand $k$ has been assigned the full rate from all the smaller bins (any $i < b$).}
%	\cradd{If $\mathbf{f^{*}}$ is the optimal solution to \eqnref{eq:geobinning}, for any flow $k$ and any two bins with index $i$ and $j$ such that $i < j$, if the allocated rate to the flow on bin $j$ is positive ($f^{*}_{kj} > 0$), the allocated rate to the flow on bin $i$ should be equal to the size of the bin ($f^{*}_{ki} = (\alpha^{i} - \alpha^{i - 1}) U$).}
\end{lemma}

\begin{proof}
	\cradd{We prove by contradiction. Let $\mathbf{\hat{f}}$ show the optimal solution of GB. If \lemmaref{lemma:gb:1} does not hold, there should be two bins with indices $i$ and $b$ such that $i < b$, $\hat{f}_{kb} > 0$ and $\hat{f}_{ki} < (\alpha^{i} - \alpha^{i - 1}) \mathcal{U}$. Observe that this contradicts the optimality of $\hat{\mathbf{f}}$ since we can improve the objective by increasing the $\hat{f}_{ki}$ and decreasing the $\hat{f}_{kb}$ by the same amount (bin $i$ has a higher weight in the objective). This modified solution is still feasible since the path allocation ($\hat{f}^p_k$) and the total flow ($\hat{f}^k$) remain the same.}
\end{proof}

%\begin{lemma}
%	\label{lemma:gb:2}
%	\cradd{The optimal solution to \eqnref{eq:geobinning} only assigns resources from bin $b$ to a given demand $k$ if all the other demands have received their maximum possible rate from all the smaller bins ($i < b$)}
%\end{lemma}
%
%\begin{proof}
%	\cradd{Let $\mathbf{\hat{f}}$ be the optimal solution to \eqnref{eq:geobinning}. If \lemmaref{lemma:gb:2} is false, there should be a demand $i$ such that it does not receive its maximum rate from a bin $j$ while some other demands receive allocation from $(j + 1)$-th bin. The rest of the proof is similar to \theoremref{th:epsilonOPT} in \secref{sec:epsilonopt} and is by contradiction.}
%	
%%	\textbf{Case 1 ($\bar{f}_{kb} \geq \hat{f}_{kb})$.} In this case, we can increase the rate of all the flows in $\mathcal{D}_s$ without reducing the allocation to demand $k$. Therefore, $\mathbf{\hat{f}}$ can not be an optimal solution to \eqnref{eq:geobinning}.
%%	
%%	\textbf{Case 2 ($\bar{f}_{kb} < \hat{f}_{kb}$).}
%\end{proof} 


\begin{theorem}
	\cradd{For $\epsilon = \frac{\delta}{\sum_{e}c_e}$, the allocations from GB is never smaller by more than $\delta$ from SWAN's allocation.} 
	
\end{theorem}

\begin{proof}
	\cradd{Let $\mathbf{\hat{f}}$ and $\mathbf{\bar{f}}$ be the optimal solution of GB and SWAN respectively. We want to prove the following:}
	
	$$\max_{k \in \mathcal{D}} \bar{f}_k - \hat{f}_k \leq \delta$$
	
	\cradd{For SWAN, if a demand $k$ has an allocation $\bar{f}_k$ in $[\alpha^{b} \mathcal{U}, \alpha^{b + 1} \mathcal{U}]$, we define the flow-bin variables as following;}
	
	\begin{equation}
		\nonumber
		\bar{f}_{kj} = 
		\left\{
			\begin{array}{lr}
				\rowcolor{white}
				(\alpha^{j} - \alpha^{j - 1}) \mathcal{U} & j < b \\
				\rowcolor{white}
				\bar{f}_k - \alpha^b \mathcal{U} & j = b \\
				\rowcolor{white}
				0 & j > b
			\end{array}
		\right\}
	\end{equation}

	\cradd{SWAN's allocation with these bin-variables is a feasible solution to \eqnref{eq:geobinning}. Therefore, we have;}
	
	$$\sum_{k \in \mathcal{D}}\sum_{b=1}^{N_\beta} \epsilon^{b-1} \bar{f}_{kb} \leq \sum_{k \in \mathcal{D}}\sum_{b=1}^{N_\beta} \epsilon^{b-1} \hat{f}_{kb}$$
	
	\pooria{Need to complete this part. It should be simiar to the proof in C1.}
\end{proof}

%\begin{theorem}
%	\cradd{The single-shot optimization in~\eqnref{eq:geobinning} produces the same solution as SWAN.}
%\end{theorem}
%
%\begin{proof}
%	\cradd{It follows directly from \lemmaref{lemma:gb:1} and \lemmaref{lemma:gb:2}.}
%\end{proof}

%\cradd{We prove by contradiction. 
%In GB, for any given flow $k$, flow variable ($f_{kb}$) assigned to a bin with lower index has a higher weight in the objective.
%Therefore, for any two bins with index $i < j$, if $f_{kj} > 0$, $f_{ki}$ should be equal to its upper bound (in case of GB, it is equal to $(\alpha^{i} - \alpha^{i - 1}) U$).
%Otherwise, our solution is not optimal and we can increase the objective by keeping the total flow rate ($f_k = \sum_{b} f_{kb}$) the same while increasing the flow variable for bin $i$ and decreasing the flow variable for bin $j$. 
%%Let a flow $k$ exist such that $\alpha^{b} U \leq f_k < \alpha^{b + 1} U$ and a bin with index $j < b$ exist such that $f_{kj} < (\alpha^{j} -  \alpha^{j - 1}) U$. Now, consider a solution $\hat{f}$ such that $\hat{f}_k$ = $f_k$ but for all $j < b$, $\hat{f}_{kj}  = (\alpha^{j} - \alpha^{j - 1}) U)$. It is eas 
%}

==> texfiles/motivation_v3.tex <==
\section{Motivation and Overall Approach}
\label{sec:design}
\label{s:motivation}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.85\linewidth]{figs/motivation/msft_motivation_demand_change.eps}
	\includegraphics[width=0.85\linewidth]{figs/motivation/msft_motivation_fairness.eps}
	\includegraphics[width=0.85\linewidth]{figs/motivation/msft_motivation_efficiency.eps}
	\caption{\textbf{Slow max-min fair resource allocators lead to under-utilization and unfairness.} Results are based on a $5$ hour trace from a production WAN.}
	\label{fig:example-slow-max-min-fair}
\end{figure}
\cradd{Faster workload dynamics~\cite{Abuzaid-ncflow} and higher availability requirements~\cite{FFC} have made fast resource allocation a necessity. Operators of multi-tenant clouds further require solutions that ensure fairness and maintain efficiency~\cite{SWAN, B4}. Prior work (\eg~\cite{Abuzaid-ncflow, FFC, Narayanan-POP, Singh-RADWAN} in TE or~\cite{Gavel-Deepak} in CS) fails to meet one or multiple of these requirements.}

\crdel{The need for fast TE has become evident with increasingly faster workload dynamics (prior work~\cite{Abuzaid-ncflow} shows WAN traffic significantly changes over short time scales) and higher availability requirements. While fast solvers that optimize only for efficiency~\cite{Abuzaid-ncflow, Liu-FFC, Narayanan-POP, Singh-RADWAN} exist and adapt to such changes, operators require a solution that provides fairness, especially in multi-tenant cloud systems. More importantly, they want to be able to balance these two objectives~\cite{SWAN, B4}.}

\crdel{Solvers that meet these requirements}\cradd{Efficient and fair solvers}~\cite{SWAN, danna-practical-max-min, Gavel-Deepak} are too slow and cannot adapt to frequently changing conditions. \crdel{Today, some providers address this as follows:}If a solver is slow and can not \crdel{finish the computation}\cradd{allocate resources} within a fixed window, the \crdel{TE}\cradd{resource allocation} pipelines \cradd{in some production environments~\cite{Abuzaid-ncflow}} use the most recent previous allocation. \cradd{This solution is sub-optimal when some nodes increase their demands in the new epoch~---~they don't get enough resources and} \crdel{Using previous allocations is problematic because some nodes might increase their demand in the new epoch and, therefore, not get enough resources.}others, who request less, receive more than they need.

\begin{figure}[tb]
	\centering
	\subfigure{\includegraphics[width=0.5\linewidth]{figs/motivation/danna_swan_miss_fraction.eps}} \hfil
	\subfigure{\includegraphics[width=0.4\linewidth]{figs/motivation/num_iterations_cogentco_64x.eps}}
	\caption{\textbf{State-of-the-art approaches' ability to keep up with changing demands (left) and the number of iterations they need (right). We capture the number of windows each approach needs (left): to keep up with demands, they need to finish within a single 5-minute window.} [both use a topology with $\sim$200 nodes and $\sim$500 edges. Left captures 160 different scenarios. Right is a highly loaded scenario~\cite{Abuzaid-ncflow} -- the results on the left figure hold across all the algorithms in \sysname]}
	\label{fig:dem-change}
\end{figure}

\crdel{In~\figref{fig:example-slow-max-min-fair},} We quantify the impact of this strategy \cradd{in the TE setting} using a 5-hour trace from a production WAN \cradd{(~\figref{fig:example-slow-max-min-fair})}, which uses a 5-minute window. We observe a solver that needs two windows (10~minutes) \crdel{for computing the allocation}\cradd{to allocate resources} faces a 20\%~--~60\% reduction in fairness and a 10\%~--~30\% reduction in efficiency relative to a solver that completes within one window. \cradd{The impact is larger when traffic changes significantly}\crdel{The reduction is higher at points where traffic changes significantly}.


How often do solvers not complete in time? \crdel{In \figref{fig:dem-change},} We use traces from~\cite{Abuzaid-ncflow} to show \cradd{the distribution of the number of windows an exact solver (Danna \etal~\cite{danna-practical-max-min}) and Microsoft's approximate solver (SWAN~\cite{SWAN}) need to compute max-min fair allocations (\figref{fig:dem-change})}\crdel{the distribution of the number of windows}\crdel{needed to compute max-min fair allocations}\crdel{by an exact solver (Danna \etal~\cite{danna-practical-max-min}) and by an approximate solver deployed in a large cloud's WAN (SWAN~\cite{SWAN})}. For nearly half of the traffic trace, these solvers exceed the 5-minute window \cradd{and often need} \crdel{ requiring} 2-3 windows \crdel{' worth of computation}to finish (\figref{fig:dem-change}, left)\crdel{.This is because}: these approaches invoke expensive optimizations multiple times (\figref{fig:dem-change}, right). 

\cradd{\sysname invokes a single optimization and always completes within a single window (\figref{fig:dem-change}). Whether a one-shot optimization is faster than an iterative approach that solves multiple optimizations depends on: (a) the number of optimizations in the iterative approach; and (b) the number of variables in the one-shot optimization vs the one's in the iterative solution. LPs are polynomial in the number of variables~\cite{boyd2004convex,solvingLP}. Our one-shot optimizations are faster than prior solutions~\cite{danna-practical-max-min, SWAN, Gavel-Deepak} because we only add a small number of variables to convert the problem into one that we can solve in one-shot and because we solve only one optimization (instead of many). See~\secref{ss:expected-run-time} for a detailed analysis. }



While \crdel{our discussion has focused on} \cradd{examples here were from} TE, \crdel{we can make similar arguments for fast solvers for CS} \cradd{CS resource allocators are similar}\crdel{: fast cluster schedulers are critical for accelerating ML training at scale}~\cite{Gavel-Deepak}. We omit detailed analysis for brevity.

{\tiny
  \begin{table}[t!]
    \centering
    {\footnotesize
      \begin{tabular}{l p{2.6in}}
      \renewcommand{\arraystretch}{1.3}
        {\bf Term} & {\bf Interpretation}\\    \hline \hline
        $\mathcal{E}, \mathcal{D}, \mathcal{P}$ & sets of resources, demands and paths \\\hline
	$c_e$ & capacity of resource $e \in \mathcal{E}$\\\hline
	$\mathbf{f}, f_k^p$ & rate allocation vector and rate for demand $k$ on path $p$\\\hline
	$d_k, w_k$ & requested rate and weight for demand $k \in \mathcal{D}$\\\hline
	$r^e_k, q^p_k$ & scaling resource consumption and rate utility for demand $k$\\\hline
     \end{tabular}
    }
\caption{Notation used in our max-min fair resource allocation model. \cradd{(Further details are in \tabref{t:notation-general})}\label{t:notation}}
  \end{table}
}

\subsection{Our model}
\label{s:unified-formulation}
\cradd{We model the multi-resource max-min fair resource allocation problem as a capacitated graph where each {\em edge} is a different resource where capacities are the amount of resource available to assign, {\em paths} encode a collection of resources which we must allocate together (\eg GPU and memory) and {\em demands} request resources on a subset of paths. We support other constraints that can be posed as affine functions over graph variables (\eg \textcolor{purple}{text in maroon} below). The algorithms in \sysname will apply to any max-min fair resource allocation problem that can be specified in this model.}

Our model takes as input:
\vspace{-0.05in}
\begin{Itemize}
\item A set of resources $\mathcal{E}$ each with capacities $c_e, e \in \mathcal{E}$.
\item A set of {\em paths} $\mathcal{P}$: each path is a group of dependent resources that we must allocate together.
\item A set of demands $\mathcal{D}$ where each demand $k$:
	\begin{Itemize}
	\item Requests some rate $d_k$
	\item Has weight $w_k$ (for weighted max-min fairness)
	\item Can be routed over a set of multiple paths $P_k \in \mathcal{P}$
	\item \textcolor{purple}{Consumes $r_k^e$ of the capacity on edge $e$ for each unit rate we assign it}
	\item \textcolor{purple}{Has utility $q_k^p$ on path $p$ for each unit rate}
	\end{Itemize}
\end{Itemize}

\cradd{The max-min fair rate allocation problem assigns rates to demands such that the weighted ratios $\frac{f_k}{w_k}$ are max-min fair: we cannot increase the allocation ratio of any demand unless we decrease it for a demand that we have currently assigned a smaller value. We have the usual feasibility constraints on rates and capacities ({\sf FeasibleAlloc}, Eqn.~\ref{eq:feasible-alloc} in~\S\ref{sec:general-form}).}

It is hard to solve this model of max-min fairness because we must jointly allocate resources along multiple paths (\ie {\em groups} of {\em resources}). We show local fairness in this case does not imply global fairness and so we cannot apply single-resource solutions to this problem.

\vspace{0.05in}
\cradd{Next, we specify max-min fair rate allocation problems in traffic engineering (TE)~\cite{SWAN,B4} and cluster scheduling (CS)~\cite{Gavel-Deepak, drf, tetris} using this model. Although the edge, path, and demand terms have a natural meaning in TE, the model is broad~---~we apply it to CS to demonstrate this.}

\cradd{\parab{TE.} The actual edges in the network (such as the WAN) are the resources and demands are services that require a certain rate between nodes in the network. The TE scheme picks the paths that each demand can take. Weights can describe how the operator wants to divide the rates (e.g., split rate $2:1$ between search and ads services).}


%For the traffic engineering problem described in SWAN and B4~\cite{SWAN,B4}, the model translates as follows: The resources are actual edges on a network such as the WAN. Demands may be services that require a certain rate between nodes in the network. The allowed paths for a demand are picked by the TE scheme and weights encode desired proportional allocations (e.g., split rate $2:1$ between search and ads services).

\cradd{\parab{CS.} Each path corresponds to a server where edges are the different types of resources (\eg CPU, memory, or GPU). Demands are jobs that have a number of workers. We model heterogeneity (\eg each worker may progress at different rates on different servers) with the utility term  $q_k^p$ and scale how much of each resource the worker uses with $r_k^e$.\footnote{We can also use these terms to model similar aspects in TE.} We can support other extensions as well such as jobs that have varying resource requirements~\cite{drf,tetris}. }

%For the cluster scheduling problem described in~\cite{Gavel-Deepak}, each path may correspond to a server with edges being resources of different kinds such as CPU, memory or GPU. Demands may be a job with a certain number of workers. \cite{Gavel-Deepak} only models GPUs but other works consider a richer set of resources including CPU, memory and IO~\cite{drf,tetris}. The utility terms $q_k^p$ encode heterogeneity such as a worker progressing at different rates on different servers. We model scaling a worker's consumption of different resources using the $r_k^e$ values. Note that traffic engineering does not use the utility or consumption scaling. Other extensions are feasible as well such as modeling jobs that have workers with varying resource requirements.


\cradd{We cannot model all problems as graphs~\cite{gersht1990joint} but we are unaware of any model that is as general as ours for max-min fair resource allocation. }




\begin{comment}
{\small
	\begin{alignat}{4}
		\multispan{4}\mbox{$\displaystyle \label{eq:feasible-alloc} {\sf FeasibleAlloc}(\mathcal{V}, \mathcal{E}, \mathcal{D}, \mathcal{P}) \triangleq \big\{\mathbf{f} \mid$}&\\
		&f_k = \sum_{p \in \mathcal{P}_k} f_k^p, & \forall k \in \mathcal{D} & ~~ \text{(allocation for demand $k$)}\nonumber\\
		&f_k \leq d_k, & \forall k \in \mathcal{D} & ~~ \text{(allocation below volume)}\nonumber\\
		&\sum_{k, p \mid p \in \mathcal{P}_k, e \in p} \!\!\!\!\! r_k f_k^p \leq c_e, & \forall e \in \mathcal{E} & ~ \text{(allocation below capacity)}\nonumber\\
		&f_k^p \geq 0 & \forall p \in \mathcal{P}, k \in \mathcal{D} & ~~ \text{(non-negative allocation)}\big\}\nonumber
	\end{alignat}
}
\end{comment}


\cut{
\begin{table}[t!]
	\centering
	{\footnotesize
		\renewcommand{\arraystretch}{1.5}
		\begin{tabular}{l p{2.15in}}
			{\bf Term} & {\bf Meaning}\\
			\hline
			\hline
			$\mathbf{t}$ & sorted rate vector, $t_i$ is the $i$-th smallest rate\\
			\hline
			$N_\beta, \mathcal{D}_b$ & number of bins and set of demands in bin $b$\\	\hline
			${\ell}_b, s_b$ & boundary and slackness of bin $b$\\
			\hline
			$f_{kb}$ & rate of demand $k$ in bin $b$ \\
			\hline
			%	\hline
		\end{tabular}
	}
	\caption{Additional notation for {\sysname}. \label{t:notation-soroush}}%\pooria{Need to generalize the Table 1 notation}
\end{table}
}

\cut{
\begin{table}
	\scriptsize
	\centering
	\begin{tabular}{p{0.5in}ll} \hline
		\textbf{\textit{Allocator}} & \textbf{\textit{Properties}} & \textbf{\textit{Parameters}} \\ \hline \hline
		\textbf{Geometric} & ({\bf T}) $\alpha$-approx fairness guarantee & $\alpha$\\ 
		\textbf{Binner} & ({\bf E}) Faster than other $\alpha$-approx methods & $\epsilon$ \\ \hline \hline
		\textbf{Adaptive} & ({\bf T}) Solution in a small set containing optimal & \#iterations\\
		\textbf{Waterfiller} &  ({\bf E}) Fastest & \\ \hline\hline
		\textbf{Equi-depth} & ({\bf T}) Better than Adaptive Waterfiller & \#iterations\\ 
		\textbf{Binner} & ({\bf E}) Fairest and fast & \#bins, $\epsilon$ \\ \hline\hline
	\end{tabular}
	\caption{\cradd{The {\sysname} allocators, their properties ({\bf T}heoretical and {\bf E}mpirical), and their parameters.}}
	\label{tab:alloc_prop}
\end{table}
}


\subsection{\sysname Overview}
\label{s:sysname-overview}

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.85\linewidth]{figs/sysname_design.pdf}
	\caption{Choosing allocators (and their parameters).}
	\label{fig:design-overview}
\end{figure}
\begin{figure}[t!]
	\includegraphics{figs/decision_tree.pdf}
	\caption{An example decision process to find allocators that match a user's goals.}
	\label{fig:decision-tree}
\end{figure}


\sysname offers a suite of \textit{allocators} which produce approximate solutions for graph-based multi-resource max-min fair allocation problems. An allocator is either an algorithm or optimization (or a combination of the two) that allocates max-min fair rates that satisfy the rate and capacity constraints. 

\autoref{tab:alloc_prop} lists our allocators, their key properties and salient parameters that let the user trade-off between fairness, speed and efficiency (see~\S\ref{s:sysn-solv-engine} for more details). We have many choices here, especially for the parameters, and we can waste computational resources if we na\"{i}vely run multiple allocators in parallel.
%As the table shows, there are numerous choices, especially for the parameters, and na\"{i}vely running multiple allocators in parallel can waste computational resources.
Instead, we present a decision process to help practitioners choose an allocator that meets their requirements. The process is simple (\autoref{fig:design-overview}): we use a decision tree (\autoref{fig:decision-tree}) and a hyper-parameter search (grid-search on a small number of problems). A sensitivity analysis in~\secref{sec:eval} indicates that the decision process is robust. We do not claim any credit for this decision process but use it as evidence that choice can be simple and effective.

Intuitively, the {\sf GeometricBinner}~(\S\ref{s:oneshotopts}) is the only allocator in \sysname for which we can prove worst-case fairness guarantees: for a given $\alpha > 1$, we guarantee the allocator assigns rates to each demand within $[\alpha^{-1}, \alpha]$ times its optimal max-min fair rate. {\sf Equi-depth Binner}~(\S\ref{s:comb_ext}) is the best choice for users who prefer fairness and efficiency but do not need formal worst-case guarantees. {\sf Adaptive Waterfiller}~(\S\ref{s:genwaterfilling}) is suitable for users who prefer speed over fairness and efficiency.


==> texfiles/optmaxminallocproof.tex <==
We prove by contradiction.  
Let ${\bf t}^*$ be the optimal max-min fair allocation rate vector and ${\bf t}^\dag$ be the result obtained by solving Eqn.~\ref{eq:max_min_flow}.
If the computed rates are not optimal, there must exist at least one demand that receives a smaller allocation with Eqn.~\ref{eq:max_min_flow}.
Among such demands, let $k$ be the demand with the smallest index in ${\bf t}^\dag$.  
Thus, we have three facts:
\begin{itemize}
\item $\forall i < k, t_i^\dag = t_i^*$
\item $t_k^\dag < t_k^*$
\item $\sum_i \epsilon^i t_i^\dag \geq \sum_i \epsilon^i t_i^*$
\end{itemize}
The last fact follows from the optimal rate ${\bf t}^*$ being a feasible solution to Eqn.~\ref{eq:max_min_flow}.
Observe that the first two facts will contradict the third when $\epsilon < \frac{t_k^* - t_k^\dag}{\sum_e c_e}$ because, intuitively, the decrease in the allocation to the $k$'th demand cannot be offset in the objective of Eqn.~\ref{eq:max_min_flow} by any increase in the allocation for the other demands (whose total allocation cannot be larger than the sum of edge capacities) due to the chosen value of $\epsilon$.

In practice, we recommend setting $\epsilon = \frac{\delta}{\sum_e c_e}$ where $\delta$ is a small value and doing so guarantees that OptMaxMinAlloc will output allocations that are never smaller by more than $\delta$ from the optimal max-min fair allocations. 
